The adaptive interpolation method: A simple scheme to prove replica formulas in Bayesian inference

In recent years important progress has been achieved towards proving the validity of the replica predictions for the (asymptotic) mutual information (or "free energy") in Bayesian inference problems. The proof techniques that have emerged appear to be quite general, despite they have been worked out on a case-by-case basis. Unfortunately, a common point between all these schemes is their relatively high level of technicality. We present a new proof scheme that is quite straightforward with respect to the previous ones. We call it the adaptive interpolation method because it can be seen as an extension of the interpolation method developped by Guerra and Toninelli in the context of spin glasses, with an interpolation path that is adaptive. In order to illustrate our method we show how to prove the replica formula for three non-trivial inference problems. The first one is symmetric rank-one matrix estimation (or factorisation), which is the simplest problem considered here and the one for which the method is presented in full details. Then we generalize to symmetric tensor estimation and random linear estimation. We believe that the present method has a much wider range of applicability and also sheds new insights on the reasons for the validity of replica formulas in Bayesian inference.

==> sections/conclusion.tex <==
\section{Conclusion}\label{conclusion}

In the present paper we have provided a new form of the interpolation method that allows to derive the replica symmetric expressions for a variety of problems in a more unified and straightforward manner.

As alluded to before the 
replica formulas often allow to delimit the performance limits of message-passing 
algorithms. Indeed the variational problem provided by the replica expression is solved by a fixed point equation which exactly corresponds to the iterative equation tracking the performance of the algorithm. For many problems of interest this has been proven 
rigorously. In particular, for matrix factorisation as well as random linear estimation it has been rigorously shown that the state evolution equation almost surely tracks
the mean-square-error of the approximate message-passing (AMP) algorithm \cite{BayatiMontanari10,lassoMontanariBayati,rangan2012iterative}. An inspection of the replica solution shows that the state evolution equation exactly correspond to the fixed point equation solving the replica symmetric minimisation problem. As a consequence the region of optimality of the AMP algorithm can be determined by analysing the structure of global and local minima of the RS potential. This has been explicitly clarified for symmetric matrix factorisation in \cite{XXT} (Corollary 1.5) and random linear estimation in \cite{barbier_ieee_replicaCS} (Theorem 3.7 and Section X). 
For the general case of tensor estimation one expects similar results but to the best of our knowledge the detailed analysis has not been performed yet.



==> sections/proofs.tex <==
\section{Proofs}
%
\subsection{Proof of the identity \eqref{dHdt}} \label{proofdH}
%
We will need a useful identity which is straightforward consequence of the Bayes law. Let $\bX$, $\bX'$ be two i.i.d \emph{replicas} drawn according to the product distribution $P_{k,t;\epsilon}(\bx|\boldsymbol{\theta}) P_{k,t;\epsilon}(\bx'|\boldsymbol{\theta})$. Then for any function $g$,\footnote{This identity has been abusively called  "Nishimori identity" in the statistical physics literature. One should however note that
it is a simple consequence of Bayes formula (see e.g appendix B of \cite{barbier_ieee_replicaCS}). The 
"true" Nishimori identity \cite{Nishimori's red book} concerns models with one extra feature, namely a gauge symmetry which allows to eliminate the input signal, and the expectation over $\bS$ in \eqref{nishibasic} can therefore be dropped (see e.g. \cite{korada2009exact}).}
\begin{align}\label{nishibasic}
\EE[\langle g(\bX, \bS) \rangle_{k,t;\epsilon}] = \EE[\langle g(\bX, \bX')\rangle_{k,t;\epsilon}].
\end{align}

Let us now compute $d f_{k,t}/dt$. Starting from \eqref{intf}, \eqref{intH}
\eqref{perturb}, one obtains
%
\begin{align}
\frac{d f_{k,t;\epsilon}}{dt}&=\frac{1}{n}\mathbb{E}\Big[\Big\langle\frac{d {\cal H}_{k,t;\epsilon}(\bX;\boldsymbol{\Theta})}{dt}\Big\rangle_{k,t;\epsilon}\Big]= \frac{1}{n}\mathbb{E}\Big[\Big\langle \frac{d }{dt}h_{\rm mf}\Big(\textbf{x}, \textbf{s},\widetilde{\textbf{z}}^{(k)},\frac{K\Delta}{t\,m_{k}} \Big)+ \frac{d }{dt}h\Big(\textbf{x}, \textbf{s},{\textbf{z}}^{(k)},\frac{K\Delta}{1-t}\Big) \Big\rangle_{k,t;\epsilon}\Big]\nonumber\\
%
&= \frac{1}{nK\Delta}\mathbb{E}\Big[\Big\langle m_k\sum_{i=1}^n\Big(\frac{X_i^2}{2} - X_iS_i-\frac{X_i\widetilde Z_i^{(k)}}{2}\sqrt{\frac{K\Delta}{t\,m_k}} \Big)- \sum_{i\le j=1}^n\Big(\frac{X_i^2X_j^2}{2n} - \frac{X_iX_jS_iS_j}{n}-\frac{X_iX_j Z_{ij}^{(k)}}{2\sqrt{n}}\sqrt{\frac{K\Delta}{1-t}} \Big) \Big\rangle_{k,t;\epsilon}\Big].\nonumber
\end{align}
%
Now we integrate by part the Gaussian noise using the elementary formula $\EE_{Z}[Zf(Z)]\!=\!\EE_Z[f'(Z)]$. This leads to
%
\begin{align}
\frac{d f_{k,t;\epsilon}}{dt}&= \frac{1}{nK\Delta}\mathbb{E}\Big[\Big\langle m_k\sum_{i=1}^n\Big(\frac{X_iX_i'}{2}- X_iS_i\Big)- \sum_{i\le j=1}^n\Big(\frac{X_iX_j X_i'X_j'}{2n}- \frac{X_iX_jS_iS_j}{n} \Big) \Big\rangle_{k,t;\epsilon}\Big],
\end{align}
%
where $\bX$, $\bX'$ are two i.i.d replicas drawn according to \eqref{post}. 
{\bf mysterious sentence for me:Note that being able to perform this integration by part is the reason of the indexing of the noise variables $\{Z_{ij}^{(k)},\widetilde Z_{i}^{(k)}\}$ by the discrete time index $k$.}
An application of identity \eqref{nishibasic} then leads to
%
\begin{align}
\frac{d f_{k,t;\epsilon}}{dt}&= \frac{1}{2K\Delta}\mathbb{E}\Big[\Big\langle \frac{1}{n^2} \sum_{i\le j=1}^nX_iX_jS_iS_j -\frac{m_k}{n}\sum_{i=1}^n X_iS_i  \Big\rangle_{k,t;\epsilon}\Big] \nonumber\\
&= \frac{1}{2K\Delta}\mathbb{E}\Big[\Big\langle  \frac{1}{2n^2} \sum_{i,j=1}^n X_iX_jS_iS_j - \frac{1}{2n^2} \sum_{i=1}^n X_i^2S_i^2 -\frac{m_k}{n}\sum_{i=1}^n X_iS_i \Big\rangle_{k,t;\epsilon}\Big]. \label{last}
\end{align}
%
The Cauchy-Schwarz inequality and \eqref{nishibasic} imply that $\mathbb{E}[\langle n^{-2}\sum_{i=1}^n X_i^2S_i^2\rangle_{k,t;\epsilon}] \!=\!{\cal O}(n^{-1})$ as long as $P_0$ has bounded second and fourth bounded moments. 
Finally, expressing the two other terms in \eqref{last} with the help of the overlap $q_{\bx,\bs}\!=\!n^{-1}\sum_{i=1}^n x_is_i$ we find \eqref{dHdt}.
\QEDA
%
%
\subsection{Proof of Lemma~\ref{tinvar}} \label{prooftinvar}
%
The proof of this lemma uses another interpolation:
%
\begin{align}
\mathbb{E}[\langle q_{\bX,\bS}^{}\rangle_{k,t;\epsilon}]-\mathbb{E}[\langle q_{\bX,\bS}^{}\rangle_{k,0;\epsilon}] = \int_0^t ds 
\frac{d\,\mathbb{E}[\langle q_{\bX,\bS}^{}\rangle_{k,s;\epsilon}]}{ds} =  \int_0^t ds \mathbb{E}\Big[\Big\langle q_{\bX,\bS}^{}\Big(\frac{d{\cal H}_{k,s;\epsilon}(\bX';\boldsymbol{\Theta})}{ds} - \frac{d{\cal H}_{k,s;\epsilon}(\bX;\boldsymbol{\Theta})}{ds}\Big)\Big\rangle_{k,s;\epsilon}\Big],\label{E0Es}
\end{align}
%
where $\bX,\bX', \bX''$ etc are i.i.d replicas distributed according to \eqref{post}. The same computations as in sec.~\ref{proofdH} lead to
%
% \begin{align}
% \frac{d{\cal H}_{k,s;\epsilon}(\bx;\boldsymbol{\theta})}{ds} = \frac{m_{k}}{K\Delta}\sum_{i=1}^n\Big(\frac{x_i^2}{2} - x_is_i -\frac{1}{2}\sqrt{\frac{K\Delta}{s\,m_{k}}}x_i\widetilde z_i^{(k)} \Big) - \frac{1}{K\Delta}\sum_{i\le j=1}^n\Big(\frac{x_i^2x_j^2}{2n} - \frac{x_ix_js_is_j}{n} -\frac{1}{2}\sqrt{\frac{K\Delta}{1-s}}\frac{x_ix_j z_{ij}^{(k)}}{\sqrt{n}} \Big).
% \end{align}
% %
% Plugging this expression in \eqref{E0Es} and integrating by part the Gaussian noise variables $\{z_{ij}^{(k)}, \widetilde z_i^{(k)}\}$ one reaches
%
\begin{align}
\mathbb{E}[\langle q_{\bX,\bS}^{}\rangle_{k,t;\epsilon}] - \mathbb{E}\big[\big\langle q_{\bX,\bS}^{}\rangle_{k,0;\epsilon}] =  \frac{1}{K} \int_0^t ds \mathbb{E}\big[\big\langle q_{\bX,\bS}^{}\big(g(\bX', \bX'';\bS) - g(\bX,\bX';\bS)\big)\big\rangle_{k,s;\epsilon}\big]\label{E0Es_2}
\end{align}
%
where we have defined
%
\begin{align}
g(\bx, \bx';\bs)\defeq \frac{m_{k}}{\Delta}\sum_{i=1}^n\Big(\frac{x_ix_i'}{2} - x_is_i \Big) - \frac{1}{\Delta}\sum_{i\le j=1}^n\Big(\frac{x_ix_j x_i'x_j'}{2n}  - \frac{x_ix_js_is_j}{n} \Big).
\end{align}
%
Finally from \eqref{E0Es_2} and Cauchy-Schwarz, one obtains
%
\begin{align}
\big|\mathbb{E}[\langle q_{\bX,\bS}^{}\rangle_{k,t;\epsilon}] - \mathbb{E}[\langle q_{\bX,\bS}^{}\rangle_{k,0;\epsilon}]\big| = {\cal O}\Big(\frac{1}{K} \sqrt{\mathbb{E}\big[\big\langle q_{\bX,\bS}^2 \big\rangle_{k,s;\epsilon}\big]  \mathbb{E}\big[\big\langle g(\bX, \bX';\bS)^2 \big\rangle_{k,s;\epsilon}\big]}\Big) = {\cal O}\Big(\frac{n}{K}\Big).\label{E0Es_4}	
\end{align}
%
The last equality is true as long as the prior $P_0$ has bounded second and fourth moments. We prove this claim now. Let us start by studying $\mathbb{E}[\langle q_{\bX,\bS}^2 \rangle_{k,s;\epsilon}]$. Using Cauchy-Schwarz for the inequality and\eqref{nishibasic} for the second equality,
%
\begin{align}
\mathbb{E}\big[\big\langle q_{\bX,\bS}^2\big\rangle_{k,s;\epsilon}\big] = \frac{1}{n^2}\sum_{i,j=1}^n\mathbb{E}\big[\big\langle X_iX_jS_iS_j \big\rangle_{k,s;\epsilon}\big] \le \frac{1}{n^2}\sum_{i,j=1}^n \sqrt{\mathbb{E}\big[\big\langle X_i^2X_j^2 \big\rangle_{k,s;\epsilon}\big]\mathbb{E}\big[S_i^2S_j^2 \big] } = \frac{1}{n^2}\sum_{i,j=1}^n \mathbb{E}\big[S_i^2S_j^2 \big]={\cal O}(1), 
\label{qsmall}
\end{align}
%
where the last equality is valid for $P_0$ with bounded second and fourth moments. 
For $\mathbb{E}[\langle g(\bX, \bX';\bS)^2 \rangle_{k,s;\epsilon}]$ we proceed similarly by 
decoupling the expectations using Cauchy-Schwarz and then using \eqref{nishibasic} to make appear 
only terms depending on the signal $\bs$. At the end one finds that under these conditions for the 
moments of $P_0$, $\mathbb{E}[\langle g(\bX, \bX';\bS)^2 \rangle_{k,s;\epsilon}]\!=\!{\cal O}(n^2)$, which 
combined with \eqref{qsmall} leads the last equality of \eqref{E0Es_4} and ends the proof. $\QEDA$
%
%












